Stealing Creator's Workflow: A Creator-Inspired Agentic Framework with Iterative Feedback Loop for Improved Scientific Short-form Generation

Generating engaging, accurate short-form videos from scientific papers is challenging due to content complexity and the gap between expert authors and readers. Existing end-to-end methods often suffer from factual inaccuracies and visual artifacts, limiting their utility for scientific dissemination. To address these issues, we propose SciTalk, a novel multi-LLM agentic framework, grounding videos in various sources, such as text, figures, visual styles, and avatars. Inspired by content creators' workflows, SciTalk uses specialized agents for content summarization, visual scene planning, and text and layout editing, and incorporates an iterative feedback mechanism where video agents simulate user roles to give feedback on generated videos from previous iterations and refine generation prompts. Experimental evaluations show that SciTalk outperforms simple prompting methods in generating scientifically accurate and engaging content over the refined loop of video generation. Although preliminary results are still not yet matching human creators' quality, our framework provides valuable insights into the challenges and benefits of feedback-driven video generation. Our code, data, and generated videos will be publicly available.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> tables/eval_rubrics.tex <==
% \begin{small}
% \begin{longtable}{p{1.4cm}|p{1.5cm}|p{1.6cm}|p{6cm}}
% \toprule
% \textbf{Type} & \textbf{Evaluation Section} & \textbf{Metric} & \textbf{Description} \\ \midrule
% \endhead


% \caption{Evaluation rubrics for human, vision language model, and feedback.}
% \label{tab:agent_info}
% \end{longtable}
% \end{small}

\begin{tiny}
\begin{longtable}{p{1.1cm}|p{1.1cm}|p{1.16cm}|p{9cm}}
\toprule
\textbf{Type} & \textbf{Evaluation Section} & \textbf{Metric} & \textbf{Description} \\ \midrule
\midrule
\endhead
Human \& \newline VLM & Content Accuracy & Scientific Integrity (\textbf{SI}) & Measures how well the video adheres to the core findings of the paper without distortion \\
\cline{3-4}

 &  &  & \\
 &  & Key \newline Concept Coverage (\textbf{KCC}) & Assesses whether the video includes the main hypotheses, methods, results, and conclusions. \\
\cmidrule{2-4}

 & Clarity & Logical Flow (\textbf{LF}) & Checks if the summary follows a logical sequence (e.g., Background → Methods → Results → Conclusion). \\
\cline{3-4}

 &  &  & \\
 &  & Comprehen- \newline sibility (\textbf{C}) & Evaluates whether the explanation is understandable for a general audience while maintaining accuracy. \\
\cmidrule{2-4}

 & Visual \& Audio Sync & Scene Readability (\textbf{SR}) & Ensures that any text on screen is clear, not too dense, and easy to read. \\
\cline{3-4}

 &  &  & \\
 &  & Audio-Visual Alignment (\textbf{AVA}) & Evaluates if spoken content matches the on-screen visuals at the right moment. \\
\cmidrule{2-4}

 & Engage- \newline ment & Attention Retention (\textbf{AR}) & Predicts how well the video keeps viewers engaged throughout. \\
\cline{3-4}
 
 &  &  & \\
 &  & Pacing & Evaluates whether the video moves too fast or too slow for comprehension. \\
\cline{3-4}

 &  &  & \\
 &  & Call-to-Action Effectiveness (\textbf{CTA}) & Checks if viewers are encouraged to read the full paper or visit related resources. \\
\cline{3-4}

 &  &  & \\
 &  & Highlight Emphasis (\textbf{HE}) & Measures if key findings are properly emphasized through animation, captions, or repetition. \\
\midrule
 
Vision Language Model & Text-Based Similarity Scores &  & Text-based similarity evaluates how similar or relevant the model-generated descriptions are for different frames or compared to ground truth descriptions. \\
\midrule

Feedback & Flashtalk & Clarity & - Is the message clear and easy to follow? \\
\cline{3-4}

 &  &  & \\
 &  & Curiosity & - Does the hook immediately capture audience interest? \\
\cline{3-4}
 
 &  &  & \\
 &  & Effectiveness & - Does the flash talk motivate viewers to explore the full content? \\
\cmidrule{2-4}

 & Sceneplan & Narrative Coherence & - Does the sequence of sub-scenes follow a logical flow?
- Are transitions smooth, avoiding abrupt shifts between scenes?
- Does the structure maintain audience engagement throughout the video? \\
\cline{3-4}
 
 &  &  & \\
 &  & Timing and Pacing & - Are the durations of sub-scenes appropriately distributed?
- Do any sections feel rushed or overly extended?
- Is the pacing consistent, maintaining viewer engagement? \\
\cline{3-4}

 &  &  & \\
 &  & Visual Relevance and Clarity & - Do the selected images and visuals align with the sub-scene descriptions?
- Are there any unclear or ambiguous visual choices?
- Does each sub-scene effectively illustrate the corresponding narration? \\
\cmidrule{2-4}

 & Text & Clarity & - Are the text components clear, concise, and logically structured?
- Do they enhance scene understanding without clutter? \\
\cline{3-4}

 &  &  & \\
 &  & Key Information Coverage & - Do the extracted texts effectively summarize core ideas from the scene? \\
\cline{3-4}

 &  &  & \\
 &  & Timing and Alignment & - Are text components timed appropriately with the audio narration and visuals?
- Do the texts appear and disappear naturally to support visual storytelling? \\
\bottomrule

\caption{Evaluation rubrics for human, vision language model, and feedback.}
\label{tab:eval_rubric_all}
\end{longtable}
\end{tiny}


==> tables/feedback_metrics.tex <==
% \begin{table*}[ht]
% \centering
% \caption{
% \textbf{Feedback metric scores (1-5) on \textit{Flashtalk Agent}, \textit{Sceneplan Agent}, and \textit{Text Assistant}.}
% The table shows the feedback scores of an iteration's outputs (flashtalk, sceneplan, and text components) with a video. Higher scores indicate better performance.
% }
% \vspace{8pt}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{llccccccccc}
% \toprule
% \textbf{Paper} & \textbf{Iter} & \multicolumn{3}{c}{\textbf{Flashtalk}} & \multicolumn{3}{c}{\textbf{Sceneplan}} \multicolumn{3}{c}{\textbf{Text}} \\ 
% \cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11}
%  % & & Clarity & Curiosity & Effectiveness & Narrative \newline Coherence & Timing \& \newline Pacing & Visual \newline Relevance & Clarity & Key Info \newline Coverage & Timing \& \newline Alignment \\
%  & & Clarity & Curiosity & Effect. & NC & TP & VR & Clarity & KIC & TA \\
% \midrule
% \multirow{5}{*}{Rockslide} 
%  & 1 & 4.0 & 4.0 & 4.0 & 3.9 & 4.1 & 3.9 & 4.0 & - & - \\
%  & 2 & 4.0 & 4.0 & 4.0 & 4.0 & 4.0 & 4.0 & 4.0 & - & - \\
%  & 3 & 3.8 & 4.0 & 3.8 & 4.0 & 4.0 & 4.0 & 4.0 & - & - \\
%  & 4 & 3.8 & 4.0 & 3.8 & 4.0 & 4.0 & 4.0 & 4.0 & - & - \\
%  & 5 & 3.8 & 4.0 & 3.8 & 4.0 & 4.0 & 4.0 & 4.0 & - & - \\
% \midrule
% \multirow{5}{*}{Qwen 2.5}
%  & 1 & - & - & - & - & - & - & - & - & - \\
%  & 2 & - & - & - & - & - & - & - & - & - \\
%  & 3 & - & - & - & - & - & - & - & - & - \\
%  & 4 & - & - & - & - & - & - & - & - & - \\
%  & 5 & - & - & - & - & - & - & - & - & - \\
% \midrule
% \multirow{5}{*}{KNowNEt}
%  & 1 & - & - & - & - & - & - & - & - & - \\
%  & 2 & - & - & - & - & - & - & - & - & - \\
%  & 3 & - & - & - & - & - & - & - & - & - \\
%  & 4 & - & - & - & - & - & - & - & - & - \\
%  & 5 & - & - & - & - & - & - & - & - & - \\
% \midrule
% \multirow{5}{*}{Tuning}
%  & 1 & - & - & - & - & - & - & - & - & - \\
%  & 2 & - & - & - & - & - & - & - & - & - \\
%  & 3 & - & - & - & - & - & - & - & - & - \\
%  & 4 & - & - & - & - & - & - & - & - & - \\
%  & 5 & - & - & - & - & - & - & - & - & - \\
% \midrule
% \multirow{5}{*}{Threads}
%  & 1 & - & - & - & - & - & - & - & - & - \\
%  & 2 & - & - & - & - & - & - & - & - & - \\
%  & 3 & - & - & - & - & - & - & - & - & - \\
%  & 4 & - & - & - & - & - & - & - & - & - \\
%  & 5 & - & - & - & - & - & - & - & - & - \\
% \midrule
% \multirow{5}{*}{Dynamic}
%  & 1 & - & - & - & - & - & - & - & - & - \\
%  & 2 & - & - & - & - & - & - & - & - & - \\
%  & 3 & - & - & - & - & - & - & - & - & - \\
%  & 4 & - & - & - & - & - & - & - & - & - \\
%  & 5 & - & - & - & - & - & - & - & - & - \\
% \bottomrule
% \end{tabular}}
% \vspace{-10pt}
% \label{tab:flash_scene_eval}
% \end{table*}



\begin{table*}[ht]
\centering
\caption{
\textbf{Feedback metric scores (1-5) on \textit{Flashtalk Agent}, \textit{Sceneplan Agent}, and \textit{Text Assistant}.}
The table shows the feedback scores of an iteration's outputs (flashtalk, sceneplan, and text components) with a video. Higher scores indicate better performance.
}
\vspace{8pt}
\resizebox{\linewidth}{!}{
\begin{tabular}{llccccccccc}
\toprule
\textbf{Paper} & \textbf{Iter} & \multicolumn{3}{c}{\textbf{Flashtalk}} & \multicolumn{3}{c}{\textbf{Sceneplan}} & \multicolumn{3}{c}{\textbf{Text}} \\ 
\cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11}
 & & Clarity & Curiosity & Effect. & NC & TP & VR & Clarity & KIC & TA \\
\midrule
\multirow{5}{*}{\textsc{Rockslide}}
 & 1 & 4.0 & 4.0 & 4.0 & 3.9 & 4.1 & 3.9 & 4.0 & 4.0 & 4.0 \\
 & 2 & 4.0 & 4.0 & 4.0 & 4.0 & 4.0 & 4.0 & 4.0 & 4.0 & 4.0 \\
 & 3 & 3.8 & 4.0 & 3.8 & 4.0 & 4.0 & 4.0 & 4.0 & 4.0 & 4.0 \\
 & 4 & 4.0 & 4.0 & 4.0 & 4.0 & 4.0 & 4.0 & 4.1 & 4.0 & 4.0 \\
 & 5 & 4.0 & 4.0 & 4.0 & 4.0 & 4.0 & 4.0 & 4.0 & 4.0 & 4.0 \\
\midrule
\multirow{5}{*}{\textsc{Qwen2.5}}
 & 1 & 4.0 & - & - & 4.0 & 3.9 & 4.0 & 3.8 & 3.5 & 3.5 \\
 & 2 & 4.0 & - & - & 4.1 & 4.1 & 4.1 & 4.0 & 3.9 & 3.9 \\
 & 3 & 4.0 & - & - & 4.0 & 4.0 & 4.0 & 4.0 & 3.6 & 3.6 \\
 & 4 & 4.0 & - & 4.0 & 4.1 & 4.1 & 4.1 & 4.1 & 3.9 & 3.9 \\
 & 5 & 4.0 & - & 3.0 & 4.0 & 4.0 & 3.9 & 4.0 & 3.6 & 3.6 \\
\midrule
\multirow{5}{*}{\textsc{Knownet}}
 & 1 & 4.0 & 4.0 & 4.0 & 4.0 & 4.0 & 4.0 & 4.0 & 4.0 & 4.0 \\
 & 2 & 3.5 & 4.0 & 4.0 & 4.0 & 4.0 & 4.0 & 4.0 & 4.0 & 4.0 \\
 & 3 & 4.0 & 4.0 & 4.0 & 4.0 & 4.0 & 4.0 & 4.0 & 4.0 & 4.0 \\
 & 4 & 3.8 & 4.0 & 3.8 & 4.0 & 4.0 & 4.0 & 4.0 & 4.0 & 4.0 \\
 & 5 & 4.0 & 4.0 & 4.0 & 4.0 & 4.0 & 4.0 & 4.0 & 3.9 & 3.9 \\
\midrule
\multirow{5}{*}{\textsc{Tuning}}
 & 1 & 4.0 & 4.0 & 4.0 & 4.0 & 4.0 & 4.0 & 4.0 & 4.0 & 4.0 \\
 & 2 & 4.0 & 4.0 & 4.0 & 3.8 & 3.8 & 4.0 & 4.0 & 4.0 & 4.0 \\
 & 3 & 4.0 & 4.0 & 4.0 & 4.0 & 3.9 & 3.9 & 4.1 & 4.1 & 3.9 \\
 & 4 & 3.8 & 4.0 & 3.8 & 4.0 & 4.0 & 4.0 & 4.0 & 4.0 & 4.0 \\
 & 5 & 3.4 & 4.0 & 3.8 & 4.0 & 4.0 & 4.0 & 4.0 & 4.0 & 4.0 \\
\midrule
\multirow{5}{*}{\textsc{Threads}}
 & 1 & 3.5 & 4.5 & 4.0 & 4.0 & 4.0 & 4.0 & 4.0 & 4.0 & 4.0 \\
 & 2 & - & 4.0 & - & 3.6 & 4.0 & 3.9 & 4.0 & 4.0 & 4.0 \\
 & 3 & 3.8 & 4.0 & 3.8 & 4.0 & 4.0 & 4.0 & 4.0 & 4.0 & 4.0 \\
 & 4 & 3.6 & 4.2 & 3.8 & 4.0 & 4.0 & 4.0 & 4.0 & 4.0 & 4.0 \\
 & 5 & 4.0 & 4.0 & 4.0 & 4.0 & 4.0 & 4.0 & 4.0 & 4.0 & 4.0 \\
\midrule
\multirow{5}{*}{\textsc{Dynamic}}
 & 1 & 3.5 & 4.0 & 3.5 & 4.1 & 4.1 & 4.1 & 4.0 & 4.0 & 4.0 \\
 & 2 & 4.0 & 4.0 & 4.0 & 4.0 & 4.0 & 4.0 & 4.0 & 3.9 & 3.9 \\
 & 3 & 4.0 & 4.0 & 4.0 & 4.1 & 4.0 & 4.1 & 4.1 & 4.0 & 3.9 \\
 & 4 & 4.0 & 4.0 & 4.0 & 3.9 & 3.9 & 3.9 & 4.0 & 4.0 & 4.0 \\
 & 5 & 4.0 & 4.0 & 4.0 & 4.1 & 3.9 & 4.0 & 4.0 & 4.0 & 4.0 \\
\bottomrule
\end{tabular}}
\vspace{-10pt}
\label{tab:feedback_metric}
\end{table*}


==> tables/flashtalk_feedback_prompt.tex <==
\begin{table*}[h]
  \renewcommand{\arraystretch}{1.2} % Adjust spacing
  \small
  \begin{tabular}{p{0.9\linewidth}} % Define column width to auto-wrap
    \texttt{You are Flashtalk Feedback Agent, an advanced multi-modal evaluator specializing in assessing 1-minute curiosity-driven flash talks, which serve as engaging overviews to drive audience interest in video generation. Rate briefly using these metrics:} \\ 

    \texttt{1. Curiosity (1-5): Does the hook immediately capture audience interest?} \\
    \texttt{2. Clarity (1-5): Is the message clear and easy to follow?} \\
    \texttt{3. Effectiveness (1-5): Does the flash talk motivate viewers to explore the full content?} \\
    
    \texttt{Each metric is rated on a scale of 1 to 5, where:} \\
    \texttt{\hspace*{2em}- 1 = Poor (Significant issues, unclear or misaligned)} \\
    \texttt{\hspace*{2em}- 3 = Adequate (Somewhat effective but needs improvement)} \\
    \texttt{\hspace*{2em}- 5 = Excellent (Clear, engaging, and well-aligned)} \\

    \texttt{Your feedback should include:} \\
    \texttt{\hspace*{2em}- Strengths of the flashtalk and video.} \\
    \texttt{\hspace*{2em}- Areas for improvement in curiosity, clarity, and effectiveness.} \\
    \texttt{\hspace*{2em}- Actionable suggestions.} \\

  \end{tabular}
  \caption{System prompt used for collecting feeback for Flashtalk Generator.}\label{tab:flashtalk_feedback_prompt}
\end{table*}

==> tables/human_created_human_model_eval.tex <==
% \begin{table*}[ht]
% \centering
% \caption{
% \textbf{Comparison on between human-created and our videos with human and VLM evaluations (1-5).}
% The table shows the evaluation scores on three different videos of a paper from human VLM. First, third, and fifth iterations are selected to measure their qualitative qualities. Higher scores indicate better performance. Two people participate in the evaluation. To get the same number of evaluations from the model, we prompt with two different temperatures (0.7 and 0.9). Model scores are in parenthesis.
% }
% \vspace{8pt}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{llcccccccccc}
% \toprule
% \textbf{Paper} & \textbf{Iter} & \multicolumn{2}{c}{\textbf{Content Accuracy}} & \multicolumn{2}{c}{\textbf{Clarity}} & \multicolumn{2}{c}{\textbf{Visual Audio Sync}} & \multicolumn{4}{c}{\textbf{Engagement}} \\ 
% \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-12}
%  & & SI & KCC & LF & C & SR & AVA & AR & Pacing & CTA & HE \\
% \midrule
% \multirow{4}{*}{Query}
%  & human & & & & & & & & & &  \\
%  & 1 & & & & & & & & & &  \\
%  & 3 & & & & & & & & & &  \\
%  & 5 & & & & & & & & & &  \\
% \midrule
% \multirow{4}{*}{Context}
%  & human & & & & & & & & & &  \\
%  & 1 & & & & & & & & & &  \\
%  & 3 & & & & & & & & & &  \\
%  & 5 & & & & & & & & & &  \\
% \midrule
% \multirow{4}{*}{Speed}
%  & human & & & & & & & & & &  \\
%  & 1 & & & & & & & & & &  \\
%  & 3 & & & & & & & & & &  \\
%  & 5 & & & & & & & & & &  \\
% \bottomrule
% \end{tabular}}
% \vspace{-10pt}
% \label{tab:human_model_eval}
% \end{table*}

% \begin{table*}[ht]
% \centering
% \caption{
% \textbf{Comparison between human-created and our videos with human and VLM evaluations (1-5).}
% The table shows the evaluation scores on three different videos of a paper from human VLM. First, third, and fifth iterations are selected to measure their qualitative qualities. Higher scores indicate better performance. Two people participated in the evaluation. To get the same number of evaluations from the model, we prompt with two different temperatures (0.7 and 0.9). Model scores are in parentheses.
% }
% \vspace{8pt}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{llcccccccccc}
% \toprule
% \textbf{Paper} & \textbf{Iter} & \multicolumn{2}{c}{\textbf{Content Accuracy}} & \multicolumn{2}{c}{\textbf{Clarity}} & \multicolumn{2}{c}{\textbf{Visual Audio Sync}} & \multicolumn{4}{c}{\textbf{Engagement}} \\ 
% \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-12}
%  & & SI & KCC & LF & C & SR & AVA & AR & Pacing & CTA & HE \\
% \midrule
% \multirow{4}{*}{Query}
%  & human & 5.0 & 5.0 & 5.0 & 5.0 & 5.0 & 5.0 & 4.0 & 5.0 & 3.5 & 5.0 \\
%  & 1 & 3.0 & 4.0 & 4.0 & 3.5 & 3.0 & 3.0 & 3.5 & 3.5 & 4.0 & 3.0 \\
%  & 3 & 3.0 & 4.0 & 3.5 & 3.0 & 3.0 & 3.0 & 3.0 & 3.5 & 3.5 & 3.5 \\
%  & 5 & 4.0 & 3.0 & 2.5 & 3.5 & 2.0 & 2.5 & 2.5 & 3.0 & 3.0 & 3.0 \\
% \midrule
% \multirow{4}{*}{Context}
%  & human & 5.0 & 5.0 & 5.0 & 5.0 & 5.0 & 5.0 & 5.0 & 5.0 & 5.0 & 5.0 \\
%  & 1 & 3.0 & 3.0 & 3.5 & 3.5 & 3.0 & 3.0 & 3.5 & 4.0 & 2.5 & 3.0 \\
%  & 3 & 3.0 & 3.0 & 4.0 & 3.0 & 3.5 & 3.5 & 4.5 & 3.5 & 3.5 & 3.5 \\
%  & 5 & 3.0 & 3.0 & 3.5 & 3.5 & 3.0 & 3.0 & 3.5 & 3.5 & 4.5 & 4.0 \\
% \midrule
% \multirow{4}{*}{Speed}
%  & human & 3.0 & 3.0 & 4.5 & 5.0 & 4.5 & 5.0 & 3.5 & 4.5 & 2.5 & 4.5 \\
%  & 1 & 4.0 & 4.0 & 4.5 & 4.5 & 3.5 & 4.0 & 5.0 & 4.0 & 4.0 & 4.0 \\
%  & 3 & 4.0 & 4.0 & 4.5 & 3.5 & 3.5 & 3.5 & 4.5 & 3.5 & 4.0 & 4.5 \\
%  & 5 & 4.0 & 4.0 & 3.5 & 3.5 & 2.5 & 4.0 & 3.0 & 3.0 & 3.5 & 4.5 \\
% \bottomrule
% \end{tabular}}
% \vspace{-10pt}
% \label{tab:human_model_eval}
% \end{table*}

\begin{table*}[ht]
\centering
\caption{
\textbf{Comparison between human-created and our videos with human and VLM evaluations (1-5).}
}
\vspace{8pt}
\resizebox{\linewidth}{!}{
\begin{tabular}{llcccccccccc}
\toprule
\textbf{Paper} & \textbf{Iter} & \multicolumn{2}{c}{\textbf{Content Accuracy}} & \multicolumn{2}{c}{\textbf{Clarity}} & \multicolumn{2}{c}{\textbf{Visual Audio Sync}} & \multicolumn{4}{c}{\textbf{Engagement}} \\ 
\cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-12}
 & & SI & KCC & LF & C & SR & AVA & AR & Pacing & CTA & HE \\
\midrule
\multirow{4}{*}{Query}
 & human & 5.0 (3.0) & 5.0 (-) & 5.0 (4.0) & 5.0 (-) & 5.0 (4.0) & 5.0 (-) & 4.0 (3.0) & 5.0 (3.5) & 3.5 (2.5) & 5.0 (4.0) \\
 & 1 & 3.0 (4.0) & 4.0 (4.5) & 4.0 (3.5) & 3.5 (4.0) & 3.0 (3.0) & 3.0 (4.0) & 3.5 (4.5) & 3.5 (3.5) & 4.0 (4.0) & 3.0 (4.0) \\
 & 3 & 3.0 (-) & 4.0 (-) & 3.5 (3.5) & 3.0 (4.0) & 3.0 (3.5) & 3.0 (4.0) & 3.0 (3.5) & 3.5 (3.0) & 3.5 (3.5) & 3.5 (3.5) \\
 & 5 & 4.0 (4.5) & 3.0 (4.0) & 2.5 (3.0) & 3.5 (-) & 2.0 (4.0) & 2.5 (4.0) & 2.5 (3.0) & 3.0 (4.0) & 3.0 (-) & 3.0 (-) \\
\midrule
\multirow{4}{*}{Context}
 & human & 5.0 (4.0) & 5.0 (4.0) & 5.0 (3.0) & 5.0 (4.0) & 5.0 (3.0) & 5.0 (4.0) & 5.0 (3.0) & 5.0 (3.0) & 5.0 (4.0) & 5.0 (4.0) \\
 & 1 & 3.0 (4.0) & 3.0 (-) & 3.5 (3.0) & 3.5 (4.0) & 3.0 (4.0) & 3.0 (3.0) & 3.5 (4.0) & 4.0 (3.0) & 2.5 (3.0) & 3.0 (2.5) \\
 & 3 & 3.0 (3.0) & 3.0 (4.0) & 4.0 (2.5) & 3.0 (4.0) & 3.5 (3.0) & 3.5 (3.0) & 4.5 (4.0) & 3.5 (3.0) & 3.5 (4.0) & 3.5 (4.0) \\
 & 5 & 3.0 (4.0) & 3.0 (-) & 3.5 (4.0) & 3.5 (5.0) & 3.0 (3.0) & 3.0 (3.5) & 3.5 (3.0) & 3.5 (4.0) & 4.5 (2.0) & 4.0 (3.0) \\
\midrule
\multirow{4}{*}{Speed}
 & human & 3.0 (3.5) & 3.0 (4.0) & 4.5 (4.0) & 5.0 (4.0) & 4.5 (3.0) & 5.0 (4.0) & 3.5 (4.0) & 4.5 (4.0) & 2.5 (4.0) & 4.5 (3.5) \\
 & 1 & 4.0 (4.0) & 4.0 (-) & 4.5 (2.5) & 4.5 (3.5) & 3.5 (3.5) & 4.0 (2.5) & 5.0 (4.0) & 4.0 (4.0) & 4.0 (2.5) & 4.0 (5.0) \\
 & 3 & 4.0 (4.0) & 4.0 (4.5) & 4.5 (4.0) & 3.5 (3.5) & 3.5 (3.5) & 3.5 (3.5) & 4.5 (4.0) & 3.5 (4.0) & 4.0 (2.5) & 4.5 (3.0) \\
 & 5 & 4.0 (3.5) & 4.0 (4.0) & 3.5 (4.0) & 3.5 (4.0) & 2.5 (2.5) & 4.0 (4.0) & 3.0 (4.0) & 3.0 (3.0) & 3.5 (3.0) & 4.5 (4.0) \\
\bottomrule
\end{tabular}}
\vspace{-10pt}
\label{tab:human_model_eval}
\end{table*}



==> tables/human_model_eval.tex <==
% template
% \begin{table*}[ht]
% \centering
% \caption{
% \textbf{Human and Vision Language Model Evaluations (1-5) on Final Videos.}
% The table shows the evaluation scores on three different videos of a paper. First, third, and fifth iterations are selected to measure their qualitative qualities. Higher scores indicate better performance. Five humans participate in the evaluation. Model scores are in parenthesis.
% }
% \vspace{8pt}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{llcccccccccc}
% \toprule
% \textbf{Paper} & \textbf{Iter} & \multicolumn{2}{c}{\textbf{Content}} & \multicolumn{2}{c}{\textbf{Readability}} & \multicolumn{2}{c}{\textbf{VAS}} & \multicolumn{4}{c}{\textbf{Engagement}} \\ 
% \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-12}
%  & & SI & KCC & LF & C & SR & AVA & AR & Pacing & CTA & HE \\
% \midrule
% \multirow{3}{*}{Rockslide}
%  & 1 & - & - & - & - & - & - & - & - & - & - \\
%  & 3 & - & - & - & - & - & - & - & - & - & - \\
%  & 5 & - & - & - & - & - & - & - & - & - & - \\
% \midrule
% \multirow{3}{*}{Qwen 2.5}
%  & 1 & - & - & - & - & - & - & - & - & - & - \\
%  & 3 & - & - & - & - & - & - & - & - & - & - \\
%  & 5 & - & - & - & - & - & - & - & - & - & - \\
% \midrule
% \multirow{3}{*}{KNowNEt}
%  & 1 & - & - & - & - & - & - & - & - & - & - \\
%  & 3 & - & - & - & - & - & - & - & - & - & - \\
%  & 5 & - & - & - & - & - & - & - & - & - & - \\
% \midrule
% \multirow{3}{*}{Tuning}
%  & 1 & - & - & - & - & - & - & - & - & - & - \\
%  & 3 & - & - & - & - & - & - & - & - & - & - \\
%  & 5 & - & - & - & - & - & - & - & - & - & - \\
% \midrule
% \multirow{3}{*}{Threads}
%  & 1 & - & - & - & - & - & - & - & - & - & - \\
%  & 3 & - & - & - & - & - & - & - & - & - & - \\
%  & 5 & - & - & - & - & - & - & - & - & - & - \\
% \midrule
% \multirow{3}{*}{Dynamic}
%  & 1 & - & - & - & - & - & - & - & - & - & - \\
%  & 3 & - & - & - & - & - & - & - & - & - & - \\
%  & 5 & - & - & - & - & - & - & - & - & - & - \\
% \midrule

% \bottomrule
% \end{tabular}}
% \vspace{-10pt}
% \label{tab:human_model_eval}
% \end{table*}

% version 1
% \begin{table*}[ht]
% \centering
% \caption{
% \textbf{Human and Vision Language Model Evaluations (1-5) on Final Videos.}
% The table shows the evaluation scores on three different videos of a paper. First, third, and fifth iterations are selected to measure their qualitative qualities. Higher scores indicate better performance. Five humans participate in the evaluation. Model scores are in parenthesis.
% }
% \vspace{8pt}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{llcccccccccc}
% \toprule
% \textbf{Paper} & \textbf{Iter} & \multicolumn{2}{c}{\textbf{Content}} & \multicolumn{2}{c}{\textbf{Readability}} & \multicolumn{2}{c}{\textbf{VAS}} & \multicolumn{4}{c}{\textbf{Engagement}} \\ 
% \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-12}
%  & & SI & KCC & LF & C & SR & AVA & AR & Pacing & CTA & HE \\
% \midrule
% \multirow{3}{*}{Rockslide}
%  & 1 & 4 & 4 & 4.5 & 4.5 & 3.5 & 2 & 3.5 & 3.5 & 4 & 4 \\
%  & 3 & 4 & 4 & 4 & 4 & 3 & 2.5 & 3.5 & 3.5 & 3.5 & 4 \\
%  & 5 & 4 & 4 & 4 & 4 & 2.5 & 3 & 2.5 & 4 & 3.5 & 4 \\
% \midrule
% \multirow{3}{*}{Qwen 2.5}
%  & 1 & 3 & 3 & 3.5 & 4 & 3 & 3 & 2.5 & 4 & 2 & 3.5 \\
%  & 3 & 4 & 4 & 3.5 & 4.5 & 3.5 & 3 & 3 & 3 & 3 & 4.5 \\
%  & 5 & 3 & 3 & 3 & 3 & 1.5 & 2 & 3 & 2.5 & 2 & 3.5 \\
% \midrule
% \multirow{3}{*}{KNowNEt}
%  & 1 & 4 & 4 & 4 & 4 & 3.5 & 3 & 3.5 & 3 & 4 & 4 \\
%  & 3 & 4 & 4 & 4 & 3 & 2 & 1 & 3 & 3.5 & 3 & 4 \\
%  & 5 & 3 & 4 & 3.5 & 3 & 1.5 & 1.5 & 3.5 & 2 & 3 & 3 \\
% \midrule
% \multirow{3}{*}{Tuning}
%  & 1 & 5 & 5 & 4 & 4.5 & 4.5 & 3.5 & 5 & 4.5 & 4 & 4.5 \\
%  & 3 & 4 & 4 & 3.5 & 3.5 & 2.5 & 2.5 & 4 & 3 & 4.5 & 3.5 \\
%  & 5 & 4 & 4 & 4.5 & 3.5 & 2 & 1.5 & 4 & 3.5 & 3.5 & 3 \\
% \midrule
% \multirow{3}{*}{Threads}
%  & 1 & 4 & 4 & 4.5 & 4 & 4 & 3.5 & 4.5 & 3.5 & 4 & 4 \\
%  & 3 & 4 & 4 & 4 & 4 & 2.5 & 2.5 & 3.5 & 3.5 & 3.5 & 4 \\
%  & 5 & 4 & 4 & 4 & 3.5 & 3 & 3 & 3.5 & 3.5 & 3 & 4.5 \\
% \midrule
% \multirow{3}{*}{Dynamic}
%  & 1 & 4 & 3 & 4 & 4.5 & 3.5 & 3.5 & 4.5 & 4 & 4.5 & 3 \\
%  & 3 & 3 & 4 & 3.5 & 3.5 & 2 & 2 & 4.5 & 3.5 & 4 & 3 \\
%  & 5 & 3 & 3 & 3 & 3.5 & 1.5 & 2 & 3 & 3.5 & 2 & 3 \\
% \bottomrule
% \end{tabular}}
% \vspace{-10pt}
% \label{tab:human_model_eval}
% \end{table*}

% version 2
% \begin{table*}[ht]
% \centering
% \caption{
% \textbf{Human and Vision Language Model Evaluations (1-5) on Final Videos.}
% The table shows the evaluation scores on three different videos of a paper. First, third, and fifth iterations are selected to measure their qualitative qualities. Higher scores indicate better performance. Five humans participate in the evaluation. Model scores are in parenthesis.
% }
% \vspace{8pt}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{llcccccccccc}
% \toprule
% \textbf{Paper} & \textbf{Iter} & \multicolumn{2}{c}{\textbf{Content}} & \multicolumn{2}{c}{\textbf{Readability}} & \multicolumn{2}{c}{\textbf{VAS}} & \multicolumn{4}{c}{\textbf{Engagement}} \\ 
% \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-12}
%  & & SI & KCC & LF & C & SR & AVA & AR & Pacing & CTA & HE \\
% \midrule
% \multirow{3}{*}{Rockslide}
%  & 1 & 4.0 & 4.0 & 4.5 & 4.5 & 3.5 & 2.0 & 3.5 & 3.5 & 4.0 & 4.0 \\
%  & 3 & 4.0 & 4.0 & 4.0 & 4.0 & 3.0 & 2.5 & 3.5 & 3.5 & 3.5 & 4.0 \\
%  & 5 & 4.0 & 4.0 & 4.0 & 4.0 & 2.5 & 3.0 & 2.5 & 4.0 & 3.5 & 4.0 \\
% \midrule
% \multirow{3}{*}{Qwen 2.5}
%  & 1 & 3.0 & 3.0 & 3.5 & 4.0 & 3.0 & 3.0 & 2.5 & 4.0 & 2.0 & 3.5 \\
%  & 3 & 4.0 & 4.0 & 3.5 & 4.5 & 3.5 & 3.0 & 3.0 & 3.0 & 3.0 & 4.5 \\
%  & 5 & 3.0 & 3.0 & 3.0 & 3.0 & 1.5 & 2.0 & 3.0 & 2.5 & 2.0 & 3.5 \\
% \midrule
% \multirow{3}{*}{KNowNEt}
%  & 1 & 4.0 & 4.0 & 4.0 & 4.0 & 3.5 & 3.0 & 3.5 & 3.0 & 4.0 & 4.0 \\
%  & 3 & 4.0 & 4.0 & 4.0 & 3.0 & 2.0 & 1.0 & 3.0 & 3.5 & 3.0 & 4.0 \\
%  & 5 & 3.0 & 4.0 & 3.5 & 3.0 & 1.5 & 1.5 & 3.5 & 2.0 & 3.0 & 3.0 \\
% \midrule
% \multirow{3}{*}{Tuning}
%  & 1 & 5.0 & 5.0 & 4.0 & 4.5 & 4.5 & 3.5 & 5.0 & 4.5 & 4.0 & 4.5 \\
%  & 3 & 4.0 & 4.0 & 3.5 & 3.5 & 2.5 & 2.5 & 4.0 & 3.0 & 4.5 & 3.5 \\
%  & 5 & 4.0 & 4.0 & 4.5 & 3.5 & 2.0 & 1.5 & 4.0 & 3.5 & 3.5 & 3.0 \\
% \midrule
% \multirow{3}{*}{Threads}
%  & 1 & 4.0 & 4.0 & 4.5 & 4.0 & 4.0 & 3.5 & 4.5 & 3.5 & 4.0 & 4.0 \\
%  & 3 & 4.0 & 4.0 & 4.0 & 4.0 & 2.5 & 2.5 & 3.5 & 3.5 & 3.5 & 4.0 \\
%  & 5 & 4.0 & 4.0 & 4.0 & 3.5 & 3.0 & 3.0 & 3.5 & 3.5 & 3.0 & 4.5 \\
% \midrule
% \multirow{3}{*}{Dynamic}
%  & 1 & 4.0 & 3.0 & 4.0 & 4.5 & 3.5 & 3.5 & 4.5 & 4.0 & 4.5 & 3.0 \\
%  & 3 & 3.0 & 4.0 & 3.5 & 3.5 & 2.0 & 2.0 & 4.5 & 3.5 & 4.0 & 3.0 \\
%  & 5 & 3.0 & 3.0 & 3.0 & 3.5 & 1.5 & 2.0 & 3.0 & 3.5 & 2.0 & 3.0 \\
% \bottomrule
% \end{tabular}}
% \vspace{-10pt}
% \label{tab:human_model_eval}
% \end{table*}

% version 3
\begin{table*}[ht]
\centering
\caption{
\textbf{Human and Vision Language Model Evaluations (1-5) on Final Videos.}
The table shows the evaluation scores on three different videos of a paper from human VLM. First, third, and fifth iterations are selected to measure their qualitative qualities. Higher scores indicate better performance. Two people participate in the evaluation. To get the same number of evaluations from the model, we prompt with two different temperatures (0.7 and 0.9). Model scores are in parenthesis.
}
\vspace{8pt}
\resizebox{\linewidth}{!}{
\begin{tabular}{llcccccccccc}
\toprule
\textbf{Paper} & \textbf{Iter} & \multicolumn{2}{c}{\textbf{Content Accuracy}} & \multicolumn{2}{c}{\textbf{Clarity}} & \multicolumn{2}{c}{\textbf{Visual Audio Sync}} & \multicolumn{4}{c}{\textbf{Engagement}} \\ 
\cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-12}
 & & SI & KCC & LF & C & SR & AVA & AR & Pacing & CTA & HE \\
\midrule
\multirow{3}{*}{Rockslide}
 & 1 & 4.0 (3.0) & 4.0 (3.5) & 4.5 (3.5) & 4.5 (4.0) & 3.5 (1.0) & 2.0 (2.0) & 3.5 (5.0) & 3.5 (3.5) & 4.0 (3.5) & 4.0 (4.0) \\
 & 3 & 4.0 (3.5) & 4.0 (4.0) & 4.0 (3.0) & 4.0 (3.0) & 3.0 (4.0) & 2.5 (4.0) & 3.5 (3.0) & 3.5 (2.0) & 3.5 (2.0) & 4.0 (3.0) \\
 & 5 & 4.0 (3.0) & 4.0 (4.0) & 4.0 (3.0) & 4.0 (4.0) & 2.5 (3.0) & 3.0 (4.0) & 2.5 (2.5) & 4.0 (3.0) & 3.5 (4.0) & 4.0 (3.5) \\
\midrule
\multirow{3}{*}{Qwen 2.5}
 & 1 & 3.0 (4.0) & 3.0 (-) & 3.5 (4.0) & 4.0 (3.0) & 3.0 (3.5) & 3.0 (3.0) & 2.5 (4.0) & 4.0 (-) & 2.0 (3.0) & 3.5 (4.0) \\
 & 3 & 4.0 (4.0) & 4.0 (-) & 3.5 (3.0) & 4.5 (4.5) & 3.5 (3.0) & 3.0 (4.0) & 3.0 (4.0) & 3.0 (3.5) & 3.0 (2.0) & 4.5 (4.0) \\
 & 5 & 3.0 (4.0) & 3.0 (4.0) & 3.0 (5.0) & 3.0 (4.0) & 1.5 (3.0) & 2.0 (4.0) & 3.0 (3.5) & 2.5 (3.5) & 2.0 (3.5) & 3.5 (3.5) \\
\midrule
\multirow{3}{*}{KNowNEt}
 & 1 & 4.0 (3.0) & 4.0 (3.5) & 4.0 (3.0) & 4.0 (3.5) & 3.5 (4.0) & 3.0 (4.0) & 3.5 (3.0) & 3.0 (4.0) & 4.0 (3.5) & 4.0 (3.5) \\
 & 3 & 4.0 (4.0) & 4.0 (3.5) & 4.0 (4.0) & 3.0 (-) & 2.0 (4.0) & 1.0 (5.0) & 3.0 (4.0) & 3.5 (3.5) & 3.0 (2.5) & 4.0 (4.5) \\
 & 5 & 3.0 (2.5) & 4.0 (3.5) & 3.5 (4.0) & 3.0 (4.0) & 1.5 (4.0) & 1.5 (3.5) & 3.5 (3.0) & 2.0 (3.0) & 3.0 (4.0) & 3.0 (3.0) \\
\midrule
\multirow{3}{*}{Tuning}
 & 1 & 5.0 (3.5) & 5.0 (3.0) & 4.0 (4.0) & 4.5 (4.0) & 4.5 (3.0) & 3.5 (3.5) & 5.0 (4.0) & 4.5 (3.0) & 4.0 (3.0) & 4.5 (3.5) \\
 & 3 & 4.0 (2.5) & 4.0 (3.0) & 3.5 (3.0) & 3.5 (4.0) & 2.5 (4.0) & 2.5 (4.0) & 4.0 (-)& 3.0 (4.0) & 4.5 (-) & 3.5 (-) \\
 & 5 & 4.0 (4.5) & 4.0 (4.0) & 4.5 (4.0) & 3.5 (3.5) & 2.0 (4.0) & 1.5 (5.0) & 4.0 (3.0) & 3.5 (3.0) & 3.5 (4.0) & 3.0 (3.0) \\
\midrule
\multirow{3}{*}{Threads}
 & 1 & 4.0 (3.5) & 4.0 (4.5) & 4.5 (3.0) & 4.0 (4.0) & 4.0 (3.5) & 3.5 (3.0) & 4.5 (4.0) & 3.5 (3.0) & 4.0 (2.0) & 4.0 (3.5) \\
 & 3 & 4.0 (4.0) & 4.0 (4.0) & 4.0 (3.0) & 4.0 (4.0) & 2.5 (2.0) & 2.5 (-) & 3.5 (4.0) & 3.5 (4.0) & 3.5 (4.0) & 4.0 (4.0) \\
 & 5 & 4.0 (3.0) & 4.0 (4.0) & 4.0 (4.0) & 3.5 (3.0) & 3.0 (4.5) & 3.0 (3.5) & 3.5 (2.0) & 3.5 (2.5) & 3.0 (2.5) & 4.5 (2.0) \\
\midrule
\multirow{3}{*}{Dynamic}
 & 1 & 4.0 (3.0) & 3.0 (3.5) & 4.0 (3.0) & 4.5 (4.0) & 3.5 (4.0) & 3.5 (3.5) & 4.5 (3.0) & 4.0 (3.0) & 4.5 (2.0) & 3.0 (-) \\
 & 3 & 3.0 (3.0) & 4.0 (4.0) & 3.5 (3.5) & 3.5 (1.0) & 2.0 (2.0) & 2.0 (3.0) & 4.5 (3.0) & 3.5 (3.0) & 4.0 (3.0) & 3.0 (4.0) \\
 & 5 & 3.0 (3.5) & 3.0 (3.5) & 3.0 (4.0) & 3.5 (2.0) & 1.5 (4.0) & 2.0 (4.5) & 3.0 (3.0) & 3.5 (4.0) & 2.0 (4.0) & 3.0 (4.0) \\
\bottomrule
\end{tabular}}
\vspace{-10pt}
\label{tab:human_model_eval}
\end{table*}

==> tables/qualitative_analysis.tex <==

% \begin{table}[h]
%     \centering
%     \begin{tabular}{|c|c|c|c|}
%         \hline
%         Paper & Iteration & Good Example & Bad Example \\ 
%         \hline
        
%         \textbf{Rockslide} &
%         1 &
%         \includegraphics[width=0.2\linewidth]{frames/A_rockslide-generated_tsunami_in_a_Greenland_fjordrang_Earth_for_9_days.pdf/2.4-good-frame-25.jpg} &
%         \includegraphics[width=0.2\linewidth]{frames/A_rockslide-generated_tsunami_in_a_Greenland_fjordrang_Earth_for_9_days.pdf/2.4-bad-frame-5.jpg} \\
%         \hline
%         \textbf{Rockslide} &
%         5 &
%         \includegraphics[width=0.2\linewidth]{frames/A_rockslide-generated_tsunami_in_a_Greenland_fjordrang_Earth_for_9_days.pdf/2.4_f0.13_multiple_rock-good-frame-101.jpg} &
%         \includegraphics[width=0.2\linewidth]{frames/A_rockslide-generated_tsunami_in_a_Greenland_fjordrang_Earth_for_9_days.pdf/2.4_f0.13_multiple_rock-bad-frame-50.jpg} \\
%         \hline
        
%         \textbf{Qwen} &
%         1 &
%         \includegraphics[width=0.2\linewidth]{frames/Qwen2.5_Technical_Report.pdf/2.3-good-frame-53.jpg} &
%         \includegraphics[width=0.2\linewidth]{frames/Qwen2.5_Technical_Report.pdf/2.3-bad-frame-89.jpg} \\
%         \hline
%         \textbf{Qwen} &
%         5 &
%         \includegraphics[width=0.2\linewidth]{frames/Qwen2.5_Technical_Report.pdf/2.3_f0.13_multiple-good-frame-88.jpg} &
%         \includegraphics[width=0.2\linewidth]{frames/Qwen2.5_Technical_Report.pdf/2.3_f0.13_multiple-bad-frame-0.jpg} \\
%         \hline
        
%         \textbf{KNowNEt} &
%         1 &
%         \includegraphics[width=0.2\linewidth]{frames/KNowNEt-Guided_Health_Information_Seeking_from_LLMs_via_Knowledge_Graph_Integration.pdf/2.4-good-frame-1.jpg} &
%         \includegraphics[width=0.2\linewidth]{frames/KNowNEt-Guided_Health_Information_Seeking_from_LLMs_via_Knowledge_Graph_Integration.pdf/2.4-bad-frame-13.jpg} \\
%         \hline
%         \textbf{KNowNEt} &
%         5 &
%         \includegraphics[width=0.2\linewidth]{frames/KNowNEt-Guided_Health_Information_Seeking_from_LLMs_via_Knowledge_Graph_Integration.pdf/2.4_f0.13_multiple_know-good-frame-0.jpg} &
%         \includegraphics[width=0.2\linewidth]{frames/KNowNEt-Guided_Health_Information_Seeking_from_LLMs_via_Knowledge_Graph_Integration.pdf/2.4_f0.13_multiple_know-bad-frame-100.jpg} \\
%         \hline

%         \textbf{Tuning} &
%         1 &
%         \includegraphics[width=0.2\linewidth]{frames/Tuning_Large_Multimodal_Models_for_Videos_using_Reinforcement_Learning_from_AI_Feedback.pdf/2.4-good-frame-41.jpg} &
%         \includegraphics[width=0.2\linewidth]{frames/Tuning_Large_Multimodal_Models_for_Videos_using_Reinforcement_Learning_from_AI_Feedback.pdf/2.4-bad-frame-6.jpg} \\
%         \hline
%         \textbf{Tuning} &
%         5 &
%         \includegraphics[width=0.2\linewidth]{frames/Tuning_Large_Multimodal_Models_for_Videos_using_Reinforcement_Learning_from_AI_Feedback.pdf/2.4_f0.13_multiple_tuning-good-frame-46.jpg} &
%         \includegraphics[width=0.2\linewidth]{frames/Tuning_Large_Multimodal_Models_for_Videos_using_Reinforcement_Learning_from_AI_Feedback.pdf/2.4_f0.13_multiple_tuning-bad-frame-76.jpg} \\
%         \hline

%         \textbf{Threads} &
%         1 &
%         \includegraphics[width=0.2\linewidth]{frames/Threads_of_Subtlety-_Detecting_Machine-Generated_Texts_Through_Discourse_Motifs.pdf/2.4-good-frame-7.jpg} &
%         \includegraphics[width=0.2\linewidth]{frames/Threads_of_Subtlety-_Detecting_Machine-Generated_Texts_Through_Discourse_Motifs.pdf/2.4-bad-frame-0.jpg} \\
%         \hline
%         \textbf{Threads} &
%         5 &
%         \includegraphics[width=0.2\linewidth]{frames/Threads_of_Subtlety-_Detecting_Machine-Generated_Texts_Through_Discourse_Motifs.pdf/2.4_f0.13_multiple_threads-good-frame-3.jpg} &
%         \includegraphics[width=0.2\linewidth]{frames/Threads_of_Subtlety-_Detecting_Machine-Generated_Texts_Through_Discourse_Motifs.pdf/2.4_f0.13_multiple_threads-bad-frame-77.jpg} \\
%         \hline

%         \textbf{Dynamic} &
%         1 &
%         \includegraphics[width=0.2\linewidth]{frames/Dynamic_Multi-Reward_Weighting_for_Multi-Style_Controllable_Generation.pdf/2.4-good-frame-32.jpg} &
%         \includegraphics[width=0.2\linewidth]{frames/Dynamic_Multi-Reward_Weighting_for_Multi-Style_Controllable_Generation.pdf/2.4-bad-frame-44.jpg} \\
%         \hline
%         \textbf{Dynamic} &
%         5 &
%         \includegraphics[width=0.2\linewidth]{frames/Dynamic_Multi-Reward_Weighting_for_Multi-Style_Controllable_Generation.pdf/2.4_f0.13_multiple_dynamic-good-frame-98.jpg} &
%         \includegraphics[width=0.2\linewidth]{frames/Dynamic_Multi-Reward_Weighting_for_Multi-Style_Controllable_Generation.pdf/2.4_f0.13_multiple_dynamic-bad-frame-7.jpg} \\
%         \hline
        
%     \end{tabular}
%     \caption{Good and bad examples for each paper and its versions.}
%     \label{tab:video_comparison}
% \end{table}


\begin{table}[h]
\centering
\small
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{Paper} & \multicolumn{3}{c|}{Iteration 1} & \multicolumn{3}{c|}{Iteration 5} \\
\cline{2-7}
& Good Example & Bad Example & Description & Good Example & Bad Example & Description \\
\hline
\textbf{Rockslide} &
\includegraphics[width=0.12\linewidth]{frames/A_rockslide-generated_tsunami_in_a_Greenland_fjordrang_Earth_for_9_days.pdf/2.4-good-frame-25.jpg} &
\includegraphics[width=0.12\linewidth]{frames/A_rockslide-generated_tsunami_in_a_Greenland_fjordrang_Earth_for_9_days.pdf/2.4-bad-frame-5.jpg} & 
Concise visual clarity vs. unclear visuals &
\includegraphics[width=0.12\linewidth]{frames/A_rockslide-generated_tsunami_in_a_Greenland_fjordrang_Earth_for_9_days.pdf/2.4_f0.13_multiple_rock-good-frame-101.jpg} &
\includegraphics[width=0.12\linewidth]{frames/A_rockslide-generated_tsunami_in_a_Greenland_fjordrang_Earth_for_9_days.pdf/2.4_f0.13_multiple_rock-bad-frame-50.jpg} &
Improved visual flow vs. misalignment issues \\
\hline

\textbf{Qwen} &
\includegraphics[width=0.12\linewidth]{frames/Qwen2.5_Technical_Report.pdf/2.3-good-frame-53.jpg} &
\includegraphics[width=0.12\linewidth]{frames/Qwen2.5_Technical_Report.pdf/2.3-bad-frame-89.jpg} &
Coherent representation vs. disconnected visuals &
\includegraphics[width=0.12\linewidth]{frames/Qwen2.5_Technical_Report.pdf/2.3_f0.13_multiple-good-frame-88.jpg} &
\includegraphics[width=0.12\linewidth]{frames/Qwen2.5_Technical_Report.pdf/2.3_f0.13_multiple-bad-frame-0.jpg} &
Enhanced scene consistency vs. repetitive errors \\
\hline

\textbf{KNowNEt} &
\includegraphics[width=0.12\linewidth]{frames/KNowNEt-Guided_Health_Information_Seeking_from_LLMs_via_Knowledge_Graph_Integration.pdf/2.4-good-frame-1.jpg} &
\includegraphics[width=0.12\linewidth]{frames/KNowNEt-Guided_Health_Information_Seeking_from_LLMs_via_Knowledge_Graph_Integration.pdf/2.4-bad-frame-13.jpg} &
Clear knowledge visualization vs. confusing layout &
\includegraphics[width=0.12\linewidth]{frames/KNowNEt-Guided_Health_Information_Seeking_from_LLMs_via_Knowledge_Graph_Integration.pdf/2.4_f0.13_multiple_know-good-frame-0.jpg} &
\includegraphics[width=0.12\linewidth]{frames/KNowNEt-Guided_Health_Information_Seeking_from_LLMs_via_Knowledge_Graph_Integration.pdf/2.4_f0.13_multiple_know-bad-frame-100.jpg} &
Improved integration of knowledge graphs vs. clutter \\
\hline

\textbf{Tuning} &
\includegraphics[width=0.12\linewidth]{frames/Tuning_Large_Multimodal_Models_for_Videos_using_Reinforcement_Learning_from_AI_Feedback.pdf/2.4-good-frame-41.jpg} &
\includegraphics[width=0.12\linewidth]{frames/Tuning_Large_Multimodal_Models_for_Videos_using_Reinforcement_Learning_from_AI_Feedback.pdf/2.4-bad-frame-6.jpg} &
Engaging visual narrative vs. poorly timed visuals &
\includegraphics[width=0.12\linewidth]{frames/Tuning_Large_Multimodal_Models_for_Videos_using_Reinforcement_Learning_from_AI_Feedback.pdf/2.4_f0.13_multiple_tuning-good-frame-46.jpg} &
\includegraphics[width=0.12\linewidth]{frames/Tuning_Large_Multimodal_Models_for_Videos_using_Reinforcement_Learning_from_AI_Feedback.pdf/2.4_f0.13_multiple_tuning-bad-frame-76.jpg} &
Enhanced coherence vs. repetitive misalignment \\
\hline

\textbf{Threads} &
\includegraphics[width=0.12\linewidth]{frames/Threads_of_Subtlety-_Detecting_Machine-Generated_Texts_Through_Discourse_Motifs.pdf/2.4-good-frame-7.jpg} &
\includegraphics[width=0.12\linewidth]{frames/Threads_of_Subtlety-_Detecting_Machine-Generated_Texts_Through_Discourse_Motifs.pdf/2.4-bad-frame-0.jpg} &
Consistent motif visualization vs. subtle errors &
\includegraphics[width=0.12\linewidth]{frames/Threads_of_Subtlety-_Detecting_Machine-Generated_Texts_Through_Discourse_Motifs.pdf/2.4_f0.13_multiple_threads-good-frame-3.jpg} &
\includegraphics[width=0.12\linewidth]{frames/Threads_of_Subtlety-_Detecting_Machine-Generated_Texts_Through_Discourse_Motifs.pdf/2.4_f0.13_multiple_threads-bad-frame-77.jpg} &
Improved motif clarity vs. visual confusion \\
\hline

\textbf{Dynamic} &
\includegraphics[width=0.12\linewidth]{frames/Dynamic_Multi-Reward_Weighting_for_Multi-Style_Controllable_Generation.pdf/2.4-good-frame-32.jpg} &
\includegraphics[width=0.12\linewidth]{frames/Dynamic_Multi-Reward_Weighting_for_Multi-Style_Controllable_Generation.pdf/2.4-bad-frame-44.jpg} &
Dynamic style coherence vs. visual inconsistency &
\includegraphics[width=0.12\linewidth]{frames/Dynamic_Multi-Reward_Weighting_for_Multi-Style_Controllable_Generation.pdf/2.4_f0.13_multiple_dynamic-good-frame-98.jpg} &
\includegraphics[width=0.12\linewidth]{frames/Dynamic_Multi-Reward_Weighting_for_Multi-Style_Controllable_Generation.pdf/2.4_f0.13_multiple_dynamic-bad-frame-7.jpg} &
Stronger multi-style balance vs. style confusion \\
\hline

\end{tabular}
\caption{Good and bad examples across different iterations with descriptions.}
\label{tab:video_comparison}
\end{table}

==> tables/sceneplan_feedback_prompt.tex <==
\begin{table*}[h]
  \renewcommand{\arraystretch}{1.2} % Adjust spacing
  \small
  \begin{tabular}{p{0.9\linewidth}} % Define column width to auto-wrap
    \texttt{You are a Sceneplan Feedback Agent, an expert in evaluating the structure, coherence, and effectiveness of scene sequences in short academic videos. Your role is to assess the Sceneplan generated for a 1-minute video based on a flash talk and provide detailed feedback on its alignment with the intended content and overall storytelling impact.} \\ 

    \texttt{The Sceneplan consists of multiple sections, each containing sub-scenes with descriptions, images, and duration constraints. These sub-scenes should be visually engaging, well-paced, and smoothly transitioned, ensuring a logical flow and effective communication.} \\ 

    \texttt{Evaluate the Sceneplan using the following three key metrics:} \\ 

    \texttt{1. Narrative Coherence:} \\
    \texttt{\hspace*{2em}- Does the sequence of sub-scenes follow a logical flow?} \\
    \texttt{\hspace*{2em}- Are transitions smooth, avoiding abrupt shifts between scenes?} \\
    \texttt{\hspace*{2em}- Does the structure maintain audience engagement throughout the video?} \\

    \texttt{2. Visual Relevance \& Clarity:} \\
    \texttt{\hspace*{2em}- Do the selected images and visuals align with the sub-scene descriptions?} \\
    \texttt{\hspace*{2em}- Are there any unclear or ambiguous visual choices?} \\
    \texttt{\hspace*{2em}- Does each sub-scene effectively illustrate the corresponding narration?} \\

    \texttt{3. Timing \& Pacing:} \\
    \texttt{\hspace*{2em}- Are the durations of sub-scenes appropriately distributed?} \\
    \texttt{\hspace*{2em}- Do any sections feel rushed or overly extended?} \\
    \texttt{\hspace*{2em}- Is the pacing consistent, maintaining viewer engagement?} \\
    
    \texttt{Each metric is rated on a scale of **1 to 5**, where:} \\
    \texttt{\hspace*{2em}- 1 = Poor (Significant issues, unclear or misaligned)} \\
    \texttt{\hspace*{2em}- 3 = Adequate (Somewhat effective but needs improvement)} \\
    \texttt{\hspace*{2em}- 5 = Excellent (Clear, engaging, and well-aligned)} \\

    \texttt{Your feedback should include:} \\
    \texttt{\hspace*{2em}- Strengths of the Sceneplan in terms of structure, visuals, and pacing.} \\
    \texttt{\hspace*{2em}- Areas for improvement, focusing on logical flow, clarity, and engagement.} \\
    \texttt{\hspace*{2em}- Actionable suggestions to enhance scene transitions, visual storytelling, and timing adjustments.} \\

  \end{tabular}
  \caption{System prompt used for collecting feeback for Sceneplan Generator.}\label{tab:sceneplan_feedback_prompt}
\end{table*}

==> tables/text_feedback_prompt.tex <==
\begin{table*}[h]
  \renewcommand{\arraystretch}{1.2} % Adjust spacing
  \small
  \begin{tabular}{p{0.9\linewidth}} % Define column width to auto-wrap
    \texttt{You are Text Feedback Agent, an expert evaluator for on-screen text components extracted by Text Assistant to enhance visual storytelling.} \\ 

    \texttt{Text Assistant extracts key phrases from scene descriptions to highlight main ideas clearly and cohesively, structuring them as effective on-screen text for visual storytelling.} \\ 

    \texttt{Evaluate concisely using these metrics:} \\ 

    \texttt{1. Clarity (1-5):} \\
    \texttt{\hspace*{2em}- Are the text components clear, concise, and logically structured?} \\
    \texttt{\hspace*{2em}- Do they enhance scene understanding without clutter?} \\
    \texttt{2. Key Information Coverage (1-5):} \\
    \texttt{\hspace*{2em}- Do the extracted texts effectively summarize core ideas from the scene?} \\
    \texttt{3. Timing and Alignment (1-5):} \\
    \texttt{\hspace*{2em}- Are text components timed appropriately with the audio narration and visuals?} \\
    \texttt{\hspace*{2em}- Do the texts appear and disappear naturally to support visual storytelling?} \\
    
    \texttt{Each metric is rated on a scale of 1 to 5, where:} \\
    \texttt{\hspace*{2em}- 1 = Poor (Significant issues, unclear or misaligned)} \\
    \texttt{\hspace*{2em}- 3 = Adequate (Somewhat effective but needs improvement)} \\
    \texttt{\hspace*{2em}- 5 = Excellent (Clear, engaging, and well-aligned)} \\

    \texttt{Provide brief feedback clearly highlighting:} \\
    \texttt{\hspace*{2em}- Main strengths} \\
    \texttt{\hspace*{2em}- Areas for improvement} \\
    \texttt{\hspace*{2em}- Short, actionable suggestions.} \\

  \end{tabular}
  \caption{System prompt used for collecting feeback for Text Assistant.}\label{tab:text_feedback_prompt}
\end{table*}
